A Performance Comparison of Sort and Scan Libraries for GPUs

Sorting and scanning are two fundamental primitives for constructing highly parallel algorithms. A number of libraries now provide implementations of these primitives for GPUs, but there is relatively little information about the performance of these implementations. We benchmark seven libraries for 32-bit integer scan and sort, and sorting 32-bit values by 32-bit integer keys. We show that there is a large variation in performance between the libraries, and that no one library has both optimal performance and portability.

==> wscript <==
import os
import re

out = 'build'

from waflib.Tools import tex
tex.re_tex = re.compile(r'\\(?P<type>include|bibliography|putbib|includegraphics|input|import|bringin|lstinputlisting|pgfplotstableread|pgfplotstabletypeset)(\[[^\[\]]*\])?{(?P<file>[^{}]*)}',re.M)

def options(opt):
    opt.load('tex')

def configure(conf):
    conf.load('tex')

def build(bld):
    bld(
            features = 'tex',
            type = 'pdflatex',
            outs = 'pdf',
            source = 'ssbench.tex'
    )

